Defensive Unlearning with Adversarial Training for Robust Concept Erasure in Diffusion Models

Diffusion models (DMs) have achieved remarkable success in text-to-image generation, but they also pose safety risks, such as the potential generation of harmful content and copyright violations. The techniques of machine unlearning, also known as concept erasing, have been developed to address these risks. However, these techniques remain vulnerable to adversarial prompt attacks, which can prompt DMs post-unlearning to regenerate undesired images containing concepts (such as nudity) meant to be erased. This work aims to enhance the robustness of concept erasing by integrating the principle of adversarial training (AT) into machine unlearning, resulting in the robust unlearning framework referred to as AdvUnlearn. However, achieving this effectively and efficiently is highly nontrivial. First, we find that a straightforward implementation of AT compromises DMs' image generation quality post-unlearning. To address this, we develop a utility-retaining regularization on an additional retain set, optimizing the trade-off between concept erasure robustness and model utility in AdvUnlearn. Moreover, we identify the text encoder as a more suitable module for robustification compared to UNet, ensuring unlearning effectiveness. And the acquired text encoder can serve as a plug-and-play robust unlearner for various DM types. Empirically, we perform extensive experiments to demonstrate the robustness advantage of AdvUnlearn across various DM unlearning scenarios, including the erasure of nudity, objects, and style concepts. In addition to robustness, AdvUnlearn also achieves a balanced tradeoff with model utility. To our knowledge, this is the first work to systematically explore robust DM unlearning through AT, setting it apart from existing methods that overlook robustness in concept erasing. Codes are available at: https://github.com/OPTML-Group/AdvUnlearn

==> rebuttal.tex <==
\setcounter{table}{0}
\setcounter{figure}{0}
\renewcommand{\thetable}{R\arabic{table}}
\renewcommand{\thefigure}{R\arabic{figure}}
\fontsize{10}{5}\selectfont
\newgeometry{top=0.25in, bottom=0.25in, left=0.5in, right=0.5in}





\begin{table}
\centering
    % \vspace*{-4mm}
    \caption{Evaluation of AdvUnlearn model robustness in ASR (Attack Success Rate) across various unlearning tasks (Nudity, Style, Object) under distinct attacks. A lower ASR indicates better robustness.}
    % \vspace*{-2mm}
    \setlength\tabcolsep{4.0pt}
    \footnotesize
    \resizebox{0.65\textwidth}{!}{
    \begin{tabular}{c||c|c|c|c|c|c}
    \toprule[1pt]
    \midrule
        \textbf{Attack Method} & \textbf{Nudity} & \textbf{Van Gogh} & \textbf{Church} & \textbf{Parachute} & \textbf{Tench} & \textbf{Garbage Truck} \\
    \toprule
        UnlearnDiffAtk & 21.13\% & 2\% & 6\% & 14\% & 4\% & 8\% \\
        CCE & 39.44\% & 28\% & 36\% & 48\% & 24\% & 44\% \\
        PEZ & 3.52\% & 0\% & 2\% & 0\% & 0\% & 4\% \\
        PH2P & 5.63\% & 0\% & 4\% & 0\% & 2\% & 6\% \\
    \midrule
    \bottomrule[1pt]
    \end{tabular}}
    \vspace{-2.5mm}
    \label{tab: robustness_evaluation_more_attack}
    %\vspace*{-8mm}
\end{table}


\begin{table}
\centering
    \caption{Evaluation of AdvUnlearn's robustness (in ASR) for nudity unlearning under the RAB attack with various token lengths. A lower ASR indicates better robustness.}
    \setlength\tabcolsep{4.0pt}
    \footnotesize
    \resizebox{0.25\textwidth}{!}{
    \begin{tabular}{c||c|c|c}
    \toprule[1pt]
    \midrule
        \textbf{Length} & \textbf{16} & \textbf{38} & \textbf{77} \\
    \toprule
        ASR & 2.11\% & 1.05\% & 1.05\% \\
    \midrule
    \bottomrule[1pt]
    \end{tabular}}
    \vspace{-2.5mm}
    \label{tab: nudity_unlearning_rab}
    %\vspace*{-8mm}
\end{table}


\begin{table}
\centering
    \caption{Erasure performance (measured by the generation rate under original inappropriate prompts w/o attack) for various DM unlearning methods across different scenarios (nudity, style, object). A lower generation rate indicates better erasing performance.}
    \setlength\tabcolsep{4.0pt}
    \footnotesize
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c||c|c|c|c|c|c}
    \toprule[1pt]
    \midrule
        \textbf{Task} & \textbf{Nudity} & \textbf{Van Gogh} & \textbf{Church} & \textbf{Parachute} & \textbf{Tench} & \textbf{Garbage Truck} \\
    \toprule
        AdvUnlearn & 7.75\% & 0\% & 0\% & 2\% & 0\% & 0\% \\
        ESD & 20.42\% & 2\% & 14\% & 4\% & 2\% & 2\% \\
        SPM & 54.93\% & 42\% & 44\% & 26\% & 6\% & 4\% \\
        FMN & 88.03\% & 10\% & 52\% & 46\% & 42\% & 40\% \\
    \midrule
    \bottomrule[1pt]
    \end{tabular}}
    \vspace{-2.5mm}
    \label{tab: erasure_performance}
    %\vspace*{-8mm}
\end{table}


\begin{table}
\centering
    \caption{Evaluation of utility performance for Van Gogh-Unlearned ESD and AdvUnlearn models through style classifier accuracy on 500 images generated in each of the other styles (Monet, Paul Cezanne, Andy Warhol). A higher accuracy indicates better utility on under a non-forgetting style.}
    \setlength\tabcolsep{4.0pt}
    \footnotesize
    \resizebox{0.3\textwidth}{!}{
    \begin{tabular}{c||c|c}
    \toprule[1pt]
    \midrule
        \textbf{Other Style} & \textbf{ESD} & \textbf{AdvUnlearn} \\
    \toprule
        Monet & 20.60\% & 52.40\% \\
        Paul Cezanne & 7.80\% & 90.80\% \\
        Andy Warhol & 45.60\% & 71.40\% \\
    \midrule
    \bottomrule[1pt]
    \end{tabular}}
    \vspace{-2.5mm}
    \label{tab: utility_performance_styles}
    %\vspace*{-8mm}
\end{table}



\begin{table}
\centering
    \caption{Evaluation of erasure performance (measured by the generation rate under original inappropriate prompts w/o attack as Tab.\,\ref{tab: erasure_performance}) and robustness (measured by ASR as Tab.\,\ref{tab: robustness_evaluation_more_attack}) for AdvUnlearn models in object unlearning scenarios with various sizes of prompt sets.}
    \setlength\tabcolsep{4.0pt}
    \footnotesize
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c|c||c|c|c|c}
    \toprule[1pt]
    \midrule
        \textbf{Prompt Number} & \textbf{Metric} & \textbf{Church} & \textbf{Parachute} & \textbf{Tench} & \textbf{Garbage Truck} \\
    \toprule
        50 & Erasure Performance & 0\% & 2\% & 0\% & 0\% \\
        50 & ASR & 6\% & 14\% & 4\% & 8\% \\
        150 & Erasure Performance & 0\% & 1.33\% & 0\% & 0\% \\
        150 & ASR & 5.33\% & 12.67\% & 4.67\% & 6\% \\
    \midrule
    \bottomrule[1pt]
    \end{tabular}}
    \vspace{-2.5mm}
    \label{tab: erasure_performance_robustness}
    %\vspace*{-8mm}
\end{table}



\begin{table}
\centering
    \caption{Evaluation of the erasing performance (measured by the generation rate under original inappropriate prompts w/o attack as Tab.\,\ref{tab: erasure_performance}) and the utility performance (measured by post-generation accuracy as Tab.\,\ref{tab: utility_performance_styles}) for ESD and AdvUnlearn models using object classifier over 500 images generated per object class.}
    \setlength\tabcolsep{4.0pt}
    \footnotesize
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{c||c|c|c|c}
    \toprule[1pt]
    \midrule
        \textbf{Unlearned Concept} & \textbf{[ESD] Unlearned Class} & \textbf{[ESD] Other Classes} & \textbf{[AdvUnlearn] Unlearned Class} & \textbf{[AdvUnlearn] Other Classes} \\
    \toprule
        Church & 3.4\% & 76.37\% & 0.4\% & 83.91\% \\
        Garbage Truck & 1.4\% & 66.86\% & 0\% & 87.91\% \\
        Parachute & 1.8\% & 78.26\% & 0.8\% & 86.11\% \\
        Tench & 0.6\% & 77.03\% & 0\% & 89.83\% \\
    \midrule
    \bottomrule[1pt]
    \end{tabular}}
    \vspace{-2.5mm}
    \label{tab: utility_erasure_performance_objects}
    %\vspace*{-8mm}
\end{table}



\begin{table}
\centering
    \caption{Evaluation of utility performance  for AdvUnlearn models across various unlearning scenarios (nudity, style, object) using different prompt set sizes for image generation, assessed by FID and CLIP scores.}
    \setlength\tabcolsep{4.0pt}
    \footnotesize
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{c|c||c|c|c}
    \toprule[1pt]
    \midrule
        \textbf{Prompt Number} & \textbf{Metric} & \textbf{Nudity} & \textbf{Van Gogh} & \textbf{Church} \\
    \toprule
        10k & FID & 19.34 & 16.96 & 18.06 \\
        10k & CLIP Score & 0.29 & 0.308 & 0.305 \\
        30k & FID & 19.15 & 17.03 & 17.94 \\
        30k & CLIP Score & 0.293 & 0.310 & 0.308 \\
    \midrule
    \bottomrule[1pt]
    \end{tabular}}
    \vspace{-2.5mm}
    \label{tab: utility_performance_advunlearn}
    %\vspace*{-8mm}
\end{table}



==> sections/OLD_exp_copy.tex <==
\section{Experiments}
\label{sec: exp}

In this section, we conduct experiments to showcase the superiority of our proposed {\ours} over current SOTA baseline methods. We empirically demonstrate that {\ours} effectively enhances the robustness of DM unlearning against adversarial prompt attacks in \textit{nudity},  \textit{style} and \textit{object} unlearning tasks while maintaining high image generation utility. Furthermore, we highlight several efficiency benefits of {\ours}, including its plug-and-play robustness when integrating the text encoder into different types of DMs and its compatibility with efficient configurations.

 
% In this section, we compare our proposed DM unlearning scheme, {\ours}, with state-of-the-art (SOTA) methods. Our extensive experiments demonstrate that {\ours} significantly enhances robustness against adversarial prompt attacks for \textit{nudity}, \textit{object} and \textit{style} unlearning while simultaneously maintaining high image generation utility. Additionally, we assess the plug-in unlearning performance of the robustly unlearned text encoder obtained through our method.  Finally, we examine the effects of various factors on {\ours}, including the choice of trainable modules, the composition of the retaining prompt datasets, the number of attack steps, and the regularization weight. 


\subsection{Experiment Setups}
\label{sec: exP_setup}


\paragraph{Concept-erasing tasks, datasets, and models.}
Although existing work has addressed various concept-erasing (\textit{i.e.}, DM unlearning) tasks \SL{[all relevant/baseline references]}, we categorize them into three main groups for ease of evaluation. (1) \textit{Nudity unlearning} focuses on preventing DMs from generating harmful content subject to nudity-related prompts \SL{[corresponding refs]}. (2) \textit{Style unlearning} aims to remove the influence of an artistic painting style in DM generation, which mimics the degeneration of copyrighted information such as the painting style \SL{[corresponding refs]}.
(3) \textit{Object unlearning}, akin to the previous tasks, targets the degeneration of DMs corresponding to a specific object \SL{[corresponding refs]}.
\SL{[@Yimeng, @Yihua, mention datasets, e.g., to collect the prompt set belong to the nudity concept to erase, we xxx. Retain set $\mathcal{C}_\mathrm{retain}$ choice and remark?].}
Model-wise, unless specified otherwise, the pre-trained SD (Stable Diffusion) v1.4 is utilized as the DM in concept erasing.  


\SL{[missing to refer to additional details in appendix?]}



%\noindent 
\paragraph{DM unlearning baselines.}
We include \textbf{8} {open-sourced} DM unlearning methods as our baselines: (1) \textbf{ESD} (erased stable diffusion) \citep{gandikota2023erasing}, (2) \textbf{FMN} (Forget-Me-Not) \citep{zhang2023forget}, 
(3) \textbf{AC} (ablating concepts) \citep{kumari2023ablating}, (4) \textbf{UCE} (unified concept editing) \citep{gandikota2023unified}, (5) \textbf{SalUn} (saliency unlearning) \cite{fan2023salun}, (6) \textbf{SH} (ScissorHands) \cite{wu2024scissorhands}, (7)  \textbf{ED} (EraseDiff) \cite{wu2024erasediff}, and (8) \textbf{SPM} (concept-SemiPermeable Membrane) \cite{lyu2023one}.
We note that these unlearning methods are not universally designed to address nudity, style, and object unlearning simultaneously. Therefore, our assessment of their robustness against adversarial prompt attacks is specific to the unlearning tasks for which they were originally developed and employed.

 

%By default, all unlearned DMs in our study are based on Stable Diffusion (SD) v1.4. 

%\noindent 
\paragraph{Training setups.} 
The implementation of {\ours} \eqref{eq: AT_ESD} follows Algorithm\,1 in Appx.\,\ref{appx: algorithm}.  
As demonstrated in Sec.\,\ref{sec: efficiency}, unlike existing DM unlearning methods, {\ours} specifically focuses on optimizing the text encoder within DMs.
\SL{A deeper analysis of the choice of the fine-tuning layer of the text encoder will also be presented later.}
% The default training configurations for {\ours} are as follows, unless specified otherwise. Different from existing DM unlearning methods, our adversarial training scheme for DM unlearning specifically targets the text encoder within the diffusion model. 
% For unlearning related to nudity, the entire text encoder is fine-tuned. In contrast, for object or style unlearning, only the first layer of the text encoder is fine-tuned.
\SL{
In the training phase of {\ours}, the upper-level optimization of \eqref{eq: AT_ESD} for minimizing the unlearning objective \eqref{eq:loss_regularization} is conducted over 1000 iterations. Each iteration uses a single data batch with the erasing guidance parameter $\eta = 1.0$ in \eqref{eq:esd_loss}  and a batch of $5$ retaining prompts with a utility regularization parameter of $\gamma = 0.3$ for nudity unlearning and $0.5$ for style and object unlearning.  
 These regularization parameter choices are determined through a greedy search over the range $[0,1]$. Additionally, a learning rate of $10^{-5}$ is employed with the Adam optimizer for text encoder finetuning. Each upper-level iteration comprises the lower-level attack generation, minimizing the attack objective \eqref{eq:attack} with $30$ attack steps and a step size of $10^{-3}$. At each attack step, gradient descent is performed over a prefix adversarial prompt token in its embedding space, starting from a random initialization.
}
% Adversarial training process consisting of $1000$ iterations, each using a single batch with a negative guidance strength of $1.0$, an attack step size of  $10^{-3}$, a learning rate of $10^{-5}$, and the Adam optimizer.
% Each iteration involves the optimization of an adversarial prompt token embedding. This embedding, initially randomly initialized, is optimized over 30 steps using \eqref{eq:attack}. It is then prepended to the original prompt token embeddings, forming a new input for the text encoder. The original prompt typically describes the concepts targeted for unlearning, such as `nudity'.
%Additionally, to compute the retaining regularization loss as per \eqref{eq:loss_regularization}, each iteration includes a batch of $5$ prompts sampled from our retaining prompt dataset. The weight assigned to the retaining regularization loss is $0.3$  for nudity unlearning and $0.5$ for style and object unlearning.


\noindent 
\textbf{Evaluation setups.} 
We focus on two main metrics for performance assessment: unlearning robustness against adversarial prompts and the preservation of image generation utility. 
% ==== Robustness Evaluation =====
For \textit{robustness} evaluation, we measure the attack success rate (\textbf{ASR}) of DMs in the presence of adversarial prompt attacks, where a lower ASR indicates better robustness. Unless specified otherwise, we utilize UnlearnDiffAtk \cite{zhang2023generate} for generating adversarial prompts at testing time, as it can be regarded as an unseen attack strategy different from the one \eqref{eq:attack} used in {\ours}. Detailed settings for attack evaluation are presented in \textbf{Appx.\,\ref{appx: attack_setup}}.
\SL{[move the following to appendix for attack evaluation setting]}
For the classification of generated images, we use NudeNet \citep{bedapudi2019nudenet} for nudity unlearning, a ViT-base model \citep{zhang2023generate} fine-tuned on the WikiArt dataset for style unlearning, and an ImageNet-pretrained ResNet-50 for object unlearning tasks. 
\SL{[move the above to appendix for attack evaluation setting]}
% ====== Utility Evaluation =======
For \textit{utility} evaluation, we use \textbf{FID} \cite{heusel2017gans} to assess the distributional quality of image generations. Besides, we also use \textbf{CLIP score}  \cite{hessel2021clipscore} to measure their contextual alignment with prompt descriptions.
 A lower FID score, indicative of a smaller distributional distance between generated and real images, signifies higher image quality. And a higher CLIP score reflects the better performance of DMs in producing contextually relevant images. 
To compute these utility metrics, we employ each DM to be evaluated to generate $10k$ images conditioned on $10k$ prompts, randomly sampled from the COCO caption dataset \cite{chen2015microsoft}.
 %While FID gauges the realism of generated images, the CLIP score evaluates their contextual relevance. 
% ==== More explainations for the relationship between FID and CLIP Score =====
%Typically, a proficient DM is expected to exhibit lower FID and higher CLIP scores simultaneously. 
%Furthermore, after concept unlearning, an increase in a DM's FID typically corresponds with a decrease in its CLIP score, and vice versa.
\SL{[remove the following. why needs this?]}
Therefore, for simplification and to facilitate comparisons \textit{among different methods}, we primarily focus on FID for utility evaluation.
It should be noted that in specific scenarios, specialized DMs such as DreamShaper \cite{DreamShaper} and Protogen \cite{Protogen}, which are fine-tuned to generate images in an animated style, may exhibit both high FID and CLIP scores. In these cases, a high FID indicates that the generated images do not resemble natural images. Conversely, if DMs display low CLIP scores, they are likely to also show low FID scores, suggesting these models have reduced image generation utility. Thus, for simplification and to facilitate comparisons \textit{among different settings of one method}, we primarily focus on the CLIP score for utility evaluation.




\subsection{Experiment Results}

% ======== Main Results =======
%\noindent 
\paragraph{Robustness-utility evaluation of {\ours} for \textit{nudity} unlearning.} 
\SL{[Why starting from Fig.\,\ref{fig: overview}. You should have a table here as well, Fig.\,\ref{fig: overview} can be used as an introductory figure.]}


% Refined Main Table for Nudity Unlearning 
\begin{wraptable}{r}{85mm}
    \vspace*{-4mm}
    \caption{\footnotesize{\SL{Performance overview of \textit{nudity} unlearning.}}}
    \vspace*{-2mm}
    \setlength\tabcolsep{4.0pt}
    \centering
    \footnotesize
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c||c|ccccc|c}
    \toprule[1pt]
    \midrule
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          \textbf{Metrics} \\ 
        \end{tabular}}  
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          SD v1.4 \\ 
          (Base)
        \end{tabular}} 
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          FMN \\ 
        \end{tabular}} 

        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          SPM \\ 
          
        \end{tabular}} 

        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          UCE \\ 
        \end{tabular}} 
        
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          ESD \\ 
        \end{tabular}} 
        
        
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          SalUn \\ 
        \end{tabular}} 
         
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          \cellcolor{Gray} {\ours} \\
          \cellcolor{Gray} (Ours)
        \end{tabular}} \\
        & & & & & & & \\
        \toprule
        
        ASR  ($\downarrow$)   & 100\% & 97.89\% & 91.55\%  & 79.58\% & 73.24\% &   11.27\% &  \cellcolor{Gray} 21.13\% \\
        FID   ($\downarrow$)  & 16.7 & 16.86 & 17.48 & 17.10 & 18.18 &   33.62 &  \cellcolor{Gray} 19.34 \\
        CLIP  ($\uparrow$)  &  0.311 &  0.308 & 0.310 & 0.309 & 0.302 &   0.287 &   \cellcolor{Gray} 0.290 \\
    
     \midrule
    \bottomrule[1pt]
    \end{tabular}}
    \vspace{-2.5mm}
    \label{tab: nudity_main}
    %\vspace*{-8mm}
\end{wraptable}

\SL{In \textbf{Tab.\,\ref{tab: nudity_main}}, we compare the adversarial robustness (measured by ASR) and the utility (evaluated using FID and CLIP score) of our proposed {\ours} with unlearning baselines when erasing the \textit{nudity} concept in DM generation.
For ease of presentation, we also refer to the DM post-unlearning (\textit{i.e.}, the unlearned DM) with the name of the corresponding unlearning method.
Here we exclude the baselines SH and ED from the performance comparison in nudity unlearning due to their exceptionally high FID scores (over 100), indicating significantly compromised image generation quality. Detailed results and visualizations for these unlearning baselines are provided in \textbf{Appx.\,\ref{appx: more_nudity_results}}.
As we can see, our proposal (\ours) demonstrates significantly improved ASR, with over 50\% ASR reduction compared to ESD, except for the lowest ASR achieved by SalUn.  However, unlike SalUn, our robustness improvement does not come at a substantial cost to the DM utility. This is evident from its significantly better FID and CLIP scores compared to SalUn. To complement our quantitative findings, \textbf{Fig.\,\ref{fig: visualization_for_nudity}} showcases the visualizations of the generations produced by various unlearned DMs in response to both the nudity-sensitive adversarial prompt and the nudity-irrelevant standard prompt. As observed, SalUn and {\ours} are the only unlearning methods that yield robust concept-erased DMs against adversarial attacks. Further, {\ours} preserves generation quality when faced with a benign prompt, unlike {\ours}.
}


\iffalse 
In \textbf{Fig.\,\ref{fig: overview}}, we compare the performance metrics of various unlearned diffusion models (DMs), including the Attack Success Rate (ASR) and Fréchet Inception Distance (FID). It is important to note that we exclude SH and ED from the performance comparison in nudity unlearning due to their extremely high FID scores (over 100), which compromise their ability to generate images properly. For detailed results and visualizations of these models, we direct readers to \textbf{Appx.\,\ref{appx: more_nudity_results}}. Notably, unlearned DMs can be categorized into two clusters. One cluster includes Salun, SH, and ED, which demonstrate considerable unlearning effectiveness but significantly compromise image generation utility, particularly ED and SH. Other DM unlearning methods, while maintaining better image generation utility, exhibit poor robustness against adversarial prompt attacks, with all recording ASRs above $70\%$ under attacks from UnlearnDiffAtk \cite{zhang2023generate}. In contrast, our proposed method, {\ours}, not only achieves substantial unlearning efficacy but also effectively preserves image generation utility. \textbf{Fig.\,\ref{fig: visualization_for_nudity}} illustrates the quality of images generated by various `nudity'-unlearned DMs, conditioned on text prompts related to both targeted and non-targeted unlearning concepts.
As we can see, FMN, SPM, and UCE cannot effectively erase nudity within the generated images. ESD, Salun, and {\ours} could successfully prevent the generated images from containing nudity. However, due to the aggressive unlearning strategy of SalUn, the generated images fail to align contextually with the text prompts, unlike ESD and {\ours}.
\fi 


% Main Table for Nudity Unlearning 
% \begin{table}[ht]
%     %\vspace*{-7mm}
%     \caption{\footnotesize{Performance evaluation of unlearning methods applied to the base SD v1.4 model for \textit{nudity} unlearning.}}
%     %\vspace*{-4mm}
%     \setlength\tabcolsep{4.0pt}
%     \centering
%     \footnotesize
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{c||c|ccccccc|c}
%     \toprule[1pt]
%     \midrule
%         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
%           \textbf{Metrics} \\ 
%         \end{tabular}}  
%         &
%         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
%           SD v1.4 \\ 
%           (Base)
%         \end{tabular}} 
%         &
%         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
%           ESD \\ 
%         \end{tabular}} 
%         &
%         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
%           FMN \\ 
%         \end{tabular}} 
%         &
%         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
%           UCE \\ 
%         \end{tabular}} 
%         &
%         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
%           SalUn \\ 
%         \end{tabular}} 
%         &
%         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
%           SH \\ 
          
%         \end{tabular}} 
%         &
%         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
%           ED \\ 
          
%         \end{tabular}} 
%          &
%         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
%           SPM \\ 
          
%         \end{tabular}} 
%         &
%         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
%           \cellcolor{Gray} {\ours} \\
%           \cellcolor{Gray} (Ours)
%         \end{tabular}} \\
%         & & & & & & & & & \\
%         \toprule
        
%         ASR  ($\downarrow$)   & 100\% & 73.24\% & 97.89\% & 79.58\% & 11.27\% & 7.04\% & 2.11\% & 91.55\% & \cellcolor{Gray} 21.13\% \\
%         FID   ($\downarrow$)  & 16.7 & 18.18 & 16.86 & 17.10 &  33.62 & 128.53 & 233.12 & 17.48 & \cellcolor{Gray} 19.34 \\
%         CLIP  ($\uparrow$)  &  0.311 &  0.302 & 0.308 & 0.309 & 0.287 & 0.235 & 0.180 & 0.310 &  \cellcolor{Gray} 0.290 \\
    
%      \midrule
%     \bottomrule[1pt]
%     \end{tabular}}
%     %\vspace{-2.5mm}
%     \label{tab: nudity_main}
%     %\vspace*{-8mm}
% \end{table}


\begin{figure} [t]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/nudity_main_visual.pdf}
    \caption{\footnotesize{Visualizations of generated images by unlearned DMs for \textit{nudity} unlearning.
    \SL{[This figure is not good, especially for utility. You should show adversarial prompt and standard prompt.
    ]}
    }}
    \label{fig: visualization_for_nudity}
\end{figure}


% === Main Table for Church Unlearning  =====
\begin{wraptable} {r}{85mm}
    \vspace*{-4mm}
    \caption{\footnotesize{Performance evaluation of unlearning methods applied to the base SD v1.4 model for \textit{Church} unlearning.}}
    %\vspace*{-4mm}
    \setlength\tabcolsep{4.0pt}
    \centering
    \footnotesize
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c||c|cccccc|c}
    \toprule[1pt]
    \midrule
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          \textbf{Metrics} \\ 
        \end{tabular}}  
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          SD v1.4 \\ 
          (Base)
        \end{tabular}} 
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          FMN \\ 
        \end{tabular}} 
         &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          SPM \\ 
          
        \end{tabular}} 
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          SalUn \\ 
        \end{tabular}} 
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          ESD \\ 
        \end{tabular}} 
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          ED \\ 
          
        \end{tabular}} 

        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          SH \\ 
          
        \end{tabular}} 

        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          \cellcolor{Gray} {\ours} \\
          \cellcolor{Gray} (Ours)
        \end{tabular}} \\
        & & & & & & & &  \\
        \toprule
        
        ASR  ($\downarrow$)   &  100\%  & 96\% &  94\% &  62\% & 60\% &  52\% &  6\% &  \cellcolor{Gray} \textbf{6\%} \\
        FID   ($\downarrow$)  & 16.70 & 16.49 & 16.76 & 17.38 &  20.95 &  17.46 &  68.02 &  \cellcolor{Gray} 18.06 \\
        CLIP  ($\uparrow$)  & 0.311 & 0.308 & 0.310 &  0.312 & 0.300 &  0.310 & 0.277 &   \cellcolor{Gray} 0.305 \\
    
     \midrule
    \bottomrule[1pt]
    \end{tabular}}
    \vspace{-2.5mm}
    \label{tab: church_main}
    %\vspace*{-8mm}
\end{wraptable}
\noindent 
\textbf{Robustness evaluation in \textit{object} unlearnings.}
In \textbf{Tab.\,\ref{tab: church_main}}, we compare various DM unlearning methods for 'Church' unlearning. It is evident that the trade-off between unlearning efficacy and image generation utility is less pronounced compared to 'nudity' unlearning. Methods such as Salun and ED that are aggressively effective in `nudity' unlearning exhibit only mild unlearning capabilities in object unlearning scenarios; however, SH remains aggressive. Most methods continue to prioritize good image generation utility but show poor robustness under the adversarial prompt attack of UnlearnDiffAtk. In contrast, our proposed {\ours} achieves the lowest ASR by merely fine-tuning the first layer of the text encoder within the DM, thus maintaining reasonable image generation utility.
\textbf{Fig.\,\ref{fig: visualization_for_church}} illustrates the quality of images generated by various `church'-unlearned DMs, conditioned on text prompts related to both targeted and non-targeted unlearning concepts. 
As observed, only SH and our proposed {\ours} could effectively erase the target concept `church'. Unlike SH, which achieves high unlearning efficacy at the cost of significant image quality degradation, {\ours} manages to properly remove the target concept `church' while preserving the non-target concept `snowy background' in the condition prompt. Additionally, it can generate images that are highly similar to the non-target images produced by the base model (SD v1.4).
For additional results and visualizations of object unlearning, refer to \textbf{Appx.\,\ref{appx: more_object_results}}.

\begin{figure} [t]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/church_main_visual.pdf}
    \caption{\footnotesize{Visualizations of generated images by unlearned DMs for \textit{church} unlearning.}}
    \label{fig: visualization_for_church}
\end{figure}



% ==== Main Table for Style Unlearning  =====
\begin{wraptable} {r}{85mm}
    \vspace*{-4mm}
    \caption{\footnotesize{Performance evaluation of unlearning methods applied to the base SD v1.4 model for \textit{Van Gogh} style unlearning.}}
    \vspace*{-2mm}
    \setlength\tabcolsep{4.0pt}
    \centering
    \footnotesize
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c||c|ccccc|c}
    \toprule[1pt]
    \midrule
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          \textbf{Metrics} \\ 
        \end{tabular}}  
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          SD v1.4 \\ 
          (Base)
        \end{tabular}} 
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          UCE \\ 
          
        \end{tabular}} 

         &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          SPM \\ 
          
        \end{tabular}} 
         &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          AC \\ 
        \end{tabular}} 

        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          FMN \\ 
        \end{tabular}} 
        
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          ESD \\ 
        \end{tabular}} 
        
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          \cellcolor{Gray} {\ours} \\
          \cellcolor{Gray} (Ours)
        \end{tabular}} \\
        & & & & & & &  \\
        \toprule
        
        ASR  ($\downarrow$)   & 100\%  & 96\%  &  88\%  & 72\%  &  52\% & 36\% &     \cellcolor{Gray} \textbf{2\%}  \\
        FID   ($\downarrow$)  & 16.70 & 16.31 &  16.65  & 17.50 & 16.59 & 18.71 &     \cellcolor{Gray} 16.96 \\
        CLIP  ($\uparrow$)  & 0.311 & 0.311 & 0.311 & 0.310 & 0.309 & 0.304 &  \cellcolor{Gray} 0.308  \\
    
     \midrule
    \bottomrule[1pt]
    \end{tabular}}
    \vspace{-3mm}
    \label{tab: style_main}
    %\vspace*{-8mm}
\end{wraptable}
\noindent 
\textbf{Robustness evaluation in \textit{style} unlearnings.}
In \textbf{Tab.\,\ref{tab: style_main}}, we evaluate various DM unlearning methods for the `Van Gogh' style, a highly recognizable target often selected for unlearning. Unlike `nudity' and object unlearning, the trade-off between unlearning efficacy and image generation utility is less severe in this context. Our proposed method effectively erases the `Van Gogh' style concept with minimal impact on image generation utility. 
\textbf{Fig.\,\ref{fig: visualization_for_style}} further illustrates the quality of images generated by various `Van Gogh'-unlearned diffusion models (DMs), conditioned on text prompts related to both targeted and non-targeted unlearning concepts. As observed, existing DM unlearning methods cannot successfully and completely erase the painting color schemes and brushstrokes of the target artist style to be unlearned while preserving other artist painting styles simultaneously. However, our proposed {\ours} could effectively erase the Van Gogh painting style precisely and preserve knowledge about other artist painting styles at the same time.



\begin{figure} [t]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/vangogh_main_visual.pdf}
    \caption{\footnotesize{Visualizations of generated images by unlearned DMs for \textit{Van Gogh} style unlearning.}}
    \label{fig: visualization_for_style}
\end{figure}







% \begin{wraptable} {r}{85mm}
%  \vspace*{-3mm}
%  \caption{\footnotesize{Performance evaluations of {\ours} using conventional training and AT on UNet and text encoder for \textit{nudity} unlearning.} 
%     }
%     %\vspace*{-5mm}
%     \centering
%     \footnotesize
%     \resizebox{0.6\textwidth}{!}{
%     \begin{tabular}{c||c|cc|cc}
%     \toprule[1pt]
%     \midrule
%     \multicolumn{2}{c||}{\centering \textbf{Training Scheme:}} & 
%     \multicolumn{2}{c|}{{Conventional Training}} & \multicolumn{2}{c}{{Adversarial Training}}   \\
%     \cmidrule{1-6}
%     \multicolumn{2}{c||}{\centering \textbf{Target Module:}} & UNet & Text Encoder &  UNet &  \cellcolor{Gray} Text Encoder   \\
%     \midrule
%     \multirow{3}{*}{    \begin{tabular}[c]{@{}c@{}}
%       \textbf{Metrics:} \\ 
%     \end{tabular}  } 
%     & ASR  ($\downarrow$) & 68.31\%  & 77.46\% &  64.79\% &  \cellcolor{Gray} 21.13\%  \\
%     & FID   ($\downarrow$) &  18.97  &  18.39 & 19.88  &  \cellcolor{Gray} 19.34 \\
%     & CLIP   ($\uparrow$)&  0.303  &  0.305 &  0.294  & \cellcolor{Gray} 0.290 \\
%      \midrule
%     \bottomrule[1pt]
%     \end{tabular}}
%     %\vspace{-2.5mm}
%     \label{table: AT_or_not}
%     %\vspace*{-14mm}
% \end{wraptable}




\begin{wrapfigure} {r}{60mm}
    \vspace*{-4mm}
    \centering
    \includegraphics[width=0.4\textwidth]{figs/layer_num_v2.pdf}
    \vspace{-2mm}
    \caption{\footnotesize{Performance comparison of different layers of text encoder finetuned through {\ours}.}}
     \vspace{-4mm}
    \label{fig: trainable_module}
\end{wrapfigure}
\noindent 
\textbf{DM unlearning effectiveness vs. choice of text encoder layers.} 
For text encoders within diffusion models, which are 12-layer transformers, \textbf{Fig.\,\ref{fig: trainable_module}} examines the impact of the number of trainable layers involved in finetuning for concept unlearning. Here, a layer number = $N$ indicates that the first $N$ layers are involved in the finetuning process. Initially, involving up to the first four layers gradually increases the number of trainable layers, significantly enhancing unlearning efficacy, reaching an ASR of approximately $40\%$. Continuing to increase the total number of layers beyond this point still improves efficacy, but the improvements are less pronounced. Once all $12$ layers are engaged in the unlearning process, the ASR could ultimately decrease to around $20\%$. Consequently, we select the entire text encoder as our default module for finetuning in 'nudity' unlearning.



\noindent 
\textbf{Plug-in performance of robust unlearned text encoder.}
Due to the modular nature of text encoders within DMs, unlearned text encoders can naturally serve as a plug-in unlearner for different DMs. To assess the train-free plugin concept unlearning performance, we finetune a text encoder with SD v1.4 and then evaluate the unlearning performance and image generation utility of directly replacing the original text encoder within DMs with the unlearned text encoder. As shown in \textbf{Tab.\,\ref{tab: plugin}}, we observe that when the unlearned text encoder is plugged into DMs with the same image generation preference, it achieves dramatic unlearning performance while preserving the image generation utility, as demonstrated with SD v1.4 and v1.5, both trained to generate realistic images. However, when the unlearned text encoder is plugged into DMs with different image generation preferences, such as DreamShaper \cite{DreamShaper} and Protogen \cite{Protogen}—which are finetuned to generate images in an animated style—the unlearning efficacy is somewhat reduced, yet it still manages to halve the ASR. Therefore, we can assert that the unlearned text encoder, finetuned through {\ours}, achieves effective plug-in unlearning efficacy, and their visualizations can be found in \textbf{Fig.\,\ref{fig: plugin_visualization}}. 

% ==== Plug in visualization ====
\begin{figure} [htb]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/plug_in_visual.pdf}
    \caption{\footnotesize{Visualization examples of images generated by different personalized DMs with plug-in {\ours} text encoder for \textit{nudity} unlearning.}}
    \label{fig: plugin_visualization}
\end{figure} 


% ==== Plug in Performance ====
\begin{table}[h]
 %\vspace*{-6mm}
 \caption{\footnotesize{Plug-in performance of {\ours} text encoder finetuned with SD v1.4 for \textit{nudity} unlearning.} 
    }
    %\vspace*{-3mm}
    \centering
    \footnotesize
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c||c|cc|cc|cc|cc}
    \toprule[1pt]
    \midrule
    \multicolumn{2}{c||}{\centering \textbf{DMs:}}
    & \multicolumn{2}{c|}{{SD v1.4}}
    & \multicolumn{2}{c|}{{SD v1.5}} 
    & \multicolumn{2}{c|}{{DreamShaper}}  &
    \multicolumn{2}{c}{{Protogen}} \\
    \cmidrule{1-10}
    \multicolumn{2}{c||}{\centering \textbf{Text Encoder:}} & Original & {\ours} & Original & {\ours} & Original & {\ours} & Original & {\ours}\\
    \midrule
    \multirow{3}{*}{    \begin{tabular}[c]{@{}c@{}}
      \textbf{Metrics:} \\ 
    \end{tabular}  } 
    & ASR  ($\downarrow$)  & 100\% &  21.13\% & 95.74\% & 16.20\% & 90.14\% & 61.27\% & 83.10\% & 42.96\% \\
    & FID   ($\downarrow$) & 16.70 & 19.34 & 16.86 & 19.27 & 23.01 & 27.40 &  20.63 & 24.47 \\
    & CLIP   ($\uparrow$) & 0.311 & 0.290 & 0.311 & 0.289 & 0.312 & 0.295 & 0.314 &  0.298 \\
     \midrule
    \bottomrule[1pt]
    \end{tabular}}
    %\vspace{-2.5mm}
    \label{tab: plugin}
    %\vspace*{-14mm}
\end{table}


% \begin{figure} [ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figs/plugin.pdf}
%     \caption{\footnotesize{Plug-in performance of {\ours} text encoder finetuned with SD v1.4 for \textit{nudity} unlearning.}}
%     \label{fig: plugin}
% \end{figure} 




% ====== Ablation Study Results ========

\begin{wraptable}{r}{85mm}
 %\vspace*{-4mm}
 \caption{\footnotesize{Performance evaluations of {\ours} using different retaining prompt dataset for \textit{nudity} unlearning.} 
    }
    \vspace*{-2mm}
    \centering
    \footnotesize
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c||c|cc|cc}
    \toprule[1pt]
    \midrule
    \multicolumn{2}{c||}{\centering \textbf{Source:}} & 
    \multicolumn{2}{c|}{{ImageNet}} & \multicolumn{2}{c}{{COCO Object}}   \\
    \cmidrule{1-6}
    \multicolumn{2}{c||}{\centering \textbf{LLM Prompt Filter:}} & \ding{56} & \ding{52} & \ding{56} &  \cellcolor{Gray} \ding{52}    \\
    \midrule
    \multirow{3}{*}{    \begin{tabular}[c]{@{}c@{}}
      \textbf{Metrics:} \\ 
    \end{tabular}  } 
    & ASR  ($\downarrow$) &  51.41\%  &  45.07\% &   38.03\% &  \cellcolor{Gray} \textbf{21.13}\%  \\
    & FID   ($\downarrow$) &  19.09   &   19.10  &  18.85  &  \cellcolor{Gray} 19.34 \\
    & CLIP   ($\uparrow$)&   0.301  &  0.299  &   0.293  & \cellcolor{Gray} 0.290 \\
     \midrule
    \bottomrule[1pt]
    \end{tabular}}
    \vspace{-3mm}
    \label{table: retain_dataset}
    %\vspace*{-14mm}
\end{wraptable}
\noindent 
\textbf{Retaining prompt dataset.}
Our proposed retaining loss regularization as defined in \eqref{eq:loss_regularization} is designed to mitigate the image generation utility degradation that often accompanies the introduction of adversarial training for unlearning. In \textbf{Tab.\,\ref{table: retain_dataset}}, we explore the influence of object class sources used to generate the prompt dataset with the template \textit{`a photo of [OBJECT]'}, and assess the impact of utilizing a Large Language Model (LLM) as a prompt filter to exclude prompts potentially relevant to the concept being erased. The prompt dataset contains an equal number of prompts for comparison. It is evident that the choice of object class for prompt dataset creation significantly affects the trade-off between unlearning efficacy and image generation utility. For instance, the COCO Object dataset, which comprises common object classes encountered in daily life, results in a lower trade-off and achieves higher unlearning efficacy compared to ImageNet, whose object classes are less commonly encountered in everyday scenarios. Moreover, the table also highlights the effectiveness of the LLM prompt filter, where LLM-filtered prompts used for {\ours} enhance unlearning efficacy with minimal impact on image generation utility, in contrast to the datasets created without such filtering.
 







\begin{wraptable}{r}{60mm}
 \vspace*{-4mm}
 \caption{\footnotesize{Performance evaluations of {\ours} using various adversarial prompting for \textit{nudity} unlearning.} 
    }
    %\vspace*{-3mm}
    \centering
    \footnotesize
    \resizebox{0.42\textwidth}{!}{
    \begin{tabular}{c||c|ccc}
    \toprule[1pt]
    \midrule
    \multicolumn{2}{c||}{\centering \textbf{Adversarial Prompting:}} & Replace & Add &  \cellcolor{Gray} Prefix   \\
    \midrule
    \multirow{3}{*}{    \begin{tabular}[c]{@{}c@{}}
      \textbf{Metrics:} \\ 
    \end{tabular}  } 
    & ASR  ($\downarrow$) &  36.63\% &  45.07\% &  \cellcolor{Gray} \textbf{21.13\%}  \\
    & FID   ($\downarrow$) & 19.39 & 19.60 &  \cellcolor{Gray} 19.34 \\
    & CLIP   ($\uparrow$)&  0.298 & 0.299  & \cellcolor{Gray} 0.290 \\
     \midrule
    \bottomrule[1pt]
    \end{tabular}}
    \vspace{-2.5mm}
    \label{table: attack_strategy}
    %\vspace*{-14mm}
\end{wraptable}
\noindent
\textbf{Adversarial prompting strategy.}
In \textbf{Tab.\,\ref{table: attack_strategy}}, we assess three different adversarial prompting strategies for original prompts that describe the concept to be unlearned: \ding{172} \textit{Replace}: directly replacing the original prompt with an optimized adversarial soft prompt; \ding{173} \textit{Add}: adding the optimized adversarial soft prompt to the original prompt in the token embedding space; \ding{174} \textit{Prefix}: prepending the optimized adversarial soft prompt before the original prompt. The \textit{Prefix} strategy is the default setting for our study. Our findings indicate that the \textit{Prefix} method is the most effective adversarial prompting choice, achieving the highest unlearning efficacy while maintaining comparable image generation utility relative to the other two prompt strategies.





% ====== Table: P4D attacks =======
\begin{wraptable}{r}{85mm}
    \vspace*{-4mm}
    \caption{\footnotesize{Robustness evaluation of unlearned DMs using different adversarial prompt attacks for \textit{nudity} unlearning.}}
    %\vspace*{-4mm}
    \setlength\tabcolsep{4.0pt}
    \centering
    \footnotesize
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c||ccccc|c}
    \toprule[1pt]
    \midrule
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          \textbf{Metrics} \\ 
        \end{tabular}}  
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          FMN \\ 
        \end{tabular}} 
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          SPM \\ 
          
        \end{tabular}} 
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          UCE \\ 
        \end{tabular}} 
        
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          ESD \\ 
        \end{tabular}} 
        
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          SalUn \\ 
        \end{tabular}} 
         
        &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          {\ours} \\
          (Ours)
        \end{tabular}} \\
        & & & & & &  \\
        \toprule
        
        P4D - ASR  ($\downarrow$)  & 97.89\% & 91.55\% & 75.35\% & 71.27\%  &  12.68\% &  19.72\% \\
        
        \cellcolor{Gray} UnlearnDiffAtk - ASR  ($\downarrow$)  &  \cellcolor{Gray} 97.89\% & \cellcolor{Gray} 91.55\% & \cellcolor{Gray} 79.58\% & \cellcolor{Gray}  73.24\% &   \cellcolor{Gray} 11.27\%  &  \cellcolor{Gray} 21.13\% \\
    
     \midrule
    \bottomrule[1pt]
    \end{tabular}}
    \vspace{-2.5mm}
    \label{tab: p4d_attack}
    %\vspace*{-8mm}
\end{wraptable}
\noindent 
\textbf{Influence of different attacks for evaluation.}
In \textbf{Tab.\,\ref{tab: p4d_attack}}, we compare the ASR of two adversarial prompt attacks for unlearned DMs: UnlearnDiffAtk \cite{zhang2023generate} (default choice) and P4D \cite{chin2023prompting4debugging}. Our observations reveal that in most cases, UnlearnDiffAtk achieves a higher ASR while utilizing less memory and requiring less attack time compared to P4D. Therefore, UnlearnDiffAtk is our default adversarial prompt attack for robustness evaluation of unlearned DMs.

\noindent 
\textbf{Other ablation studies.} 
In \textbf{Appx.\,\ref{appx: other_ablation}}, we demonstrate more ablation studies. This includes:
\ding{182} the impact of the utility-retaining regularization weight on {\ours} (\textbf{Fig.\,\ref{fig: regularization_weight}}); 
\ding{183} the effect of the number of attack steps on adversarial prompt generation for {\ours} (\textbf{Fig.\,\ref{fig: attack_num}}).

==> sections/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 
% v
% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In \textbf{Sec.\,\ref{sec: exp}}, through extensive experiments, we accurately reflect the contributions and scope of the paper.
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    Discussions on limitations of our work can be found in \textbf{Appx.\,\ref{appx: limitations}}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    Observing the vulnerability of existing unlearned Diffusion Models (DMs), we have systematically explored robust DM unlearning through adversarial training (AT). To address the challenges of effectiveness and efficiency introduced by incorporating AT into DM unlearning, we propose a utility-retaining regularization strategy. Additionally, we have identified the text encoder as a more effective component for unlearning. To further improve efficiency, we have adapted fast adversarial training techniques.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    Experiment setups can be found in \textbf{Sec.\,\ref{sec: exP_setup}} and \textbf{Appx.\,\ref{appx: attack_setup}}. Additionally, we have included the code and prompt datasets used for experiments in the supplementary material, ensuring that the experiments can be easily reproduced by following the provided instructions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have included the code and prompt datasets used for experiments in the supplementary material, ensuring that the experiments can be easily reproduced by following the provided instructions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Experiment setups can be found in \textbf{Sec.\,\ref{sec: exP_setup}} and \textbf{Appx.\,\ref{appx: attack_setup}}. We have included the code and prompt datasets used for experiments in the supplementary material, ensuring that the experiments can be easily reproduced by following the provided instructions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Error bars are not reported because it would be too computationally expensive.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    Details of hardware and corresponding computation time can be found in Line 861 - 873. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have made sure to preserve anonymity.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The discussion on broader impacts can be found in \textbf{Appx.\,\ref{appx: broader_impacts}}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper is designed for defensive DM unlearning.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    We cite the original paper that produced the code package and dataset.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have included the code and prompt datasets used for experiments in the supplementary material, ensuring that the experiments can be easily reproduced by following the provided instructions. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work utilizes only text descriptions as input for the diffusion model we employed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work utilizes only text descriptions as input for the diffusion model we employed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> sections/introduction.tex <==
\section{Introduction}


% === Background ===
% \SL{[The first paragraph reads quite similar to the ECCV submission. We should consider revising and updating it. This can come later once the technical part and the experiment part are revised.]}

Recent rapid advancements in diffusion models (DMs) \cite{ho2020denoising, song2019generative, song2020score, dhariwal2021diffusion, nichol2021improved, watson2021learning, rombach2022high, croitoru2023diffusion} have popularized the realm of text-to-image generation. These models, trained on extensive online datasets, can generate remarkably realistic images. 
However, their training heavily relies on diverse internet-sourced content and can introduce safety concerns when prompted with inappropriate texts, such as the generation of NSFW (Not Safe For Work) images, highlighted in several studies \cite{rando2022red,schramowski2023safe}. 
% To alleviate these risks, some methods \cite{schramowski2023safe,nichol2021glide} have incorporated NSFW safety checkers, either before or after image generation, to minimize the harmful effects of 
% such prompts.
% Nonetheless, relying solely on these external safety measures does not address the core safety issues of DMs, as these solutions are model-independent and rely on post-hoc interventions. Research has shown that these interventions are insufficient for completely preventing the generation of unsafe content \cite{ yang2023sneakyprompt}. 
To address this concern, post-hoc safety checkers were initially applied to DMs \cite{schramowski2023safe, nichol2021glide}. However, they were later found to be inadequate in effectively preventing the generation of unsafe content.
To further enhance safety, the concept of \textit{machine unlearning} (\textbf{MU}) has been introduced \cite{nguyen2022survey,shaik2023exploring,cao2015towards,thudi2022unrolling,xu2023machine,jia2023model, fan2024challenging}, aiming to mitigate the influence of undesired textual concepts in DM training or fine-tuning \cite{gandikota2023erasing,zhang2023forget,kumari2023ablating,gandikota2023unified}.
As a result, DMs post-unlearning (referred to as `unlearned DMs') are designed to negate the generation of undesirable content, even when faced with inappropriate prompts.

%These methods aim to selectively erase the influence of specific training data to enhance a model’s trustworthiness without retraining. These unlearned DMs ought to negate the generation of undesirable content even in the presence of inappropriate prompts. 

% other studies \cite{gandikota2023erasing,zhang2023forget,kumari2023ablating,gandikota2023unified} designed DM training or fine-tuning procedures, which align with the broader concept of \textit{machine unlearning} (\textbf{MU}) \cite{nguyen2022survey,shaik2023exploring,cao2015towards,thudi2022unrolling,xu2023machine,jia2023model, fan2024challenging}. These methods aim to selectively erase the influence of specific training data to enhance a model’s trustworthiness without retraining. These unlearned DMs ought to negate the generation of undesirable content even in the presence of inappropriate prompts. 

\begin{wrapfigure}{r}{58mm}
    \vspace{-1em}
    \centering
    \includegraphics[width=0.41\textwidth]{figs/nudity_main.pdf}
    \vspace*{-6mm}
    \caption{\footnotesize{Performance comparison overview for \textit{nudity} unlearning: various DM unlearning methods and our proposed {\ours}.
    }}
    \label{fig: overview}
    %\vspace{-4em}
    \vspace{-6em}
\end{wrapfigure}
However, the recent work on safety-driven unlearned diffusion models (DMs) \cite{zhang2023generate,chin2023prompting4debugging,tsai2023ring,pham2024circumventing} have revealed a significant challenge: existing DM unlearning methods are not sufficiently robust against \textit{adversarial prompt attacks}. These attacks involve crafting adversarial text tokens prepended to benign text prompts as input for the text-to-image generation task. The resulting adversarial prompts often manipulate unlearned DMs into producing images that include concepts they were supposed to forget. This vulnerability leads us to the \textbf{primary research question} of our study:
\begin{center}
\textit{\textbf{(Q)} Is there a principled approach to boost the robustness of the unlearned DMs against adversarial prompt attacks?}
\end{center}


Inspired by the successes of adversarial training (AT) \cite{madry2017towards} in bolstering resistance to adversarial attacks, our work explores the integration of AT with MU, termed {\ours}. This method integrates the adversarial soft prompts, which are optimized to induce the model to generate the undesirable contents, into the concept unlearning process in order to enhance the unlearning robustness. In the meantime, in order to retain the generation quality and mitigate the unwanted model utility loss, a utility-retaining regularization strategy is designed.

% Moreover, previous efforts \cite{gandikota2023erasing,zhang2023forget,kumari2023ablating,gandikota2023unified,huang2023receler} have focused on UNet. 
% ===== AT for DM unlearning ======
The most closely related work to ours is Receler \cite{huang2023receler}, which employs AT to train adapters within UNet for DM unlearning and introduces the use of spatial information linked to the target concept’s text tokens to regularize adapter outputs. 
% ===== Differences ======
Diverging from this approach, our study revealed that text encoders are particularly effective in boosting the robustness of DM unlearning against adversarial prompts while preserving image generation quality. Moreover, the modular nature of the text encoder supports plug-and-play fine-tuning for specific concept unlearning, thus enhancing flexibility and effectiveness across various UNets.
Additionally, our proposed utility-retaining loss regularization not only leverages extra training data but also integrates smoothly with other training losses to sustain image generation utility. We further explore the feasibility of substituting traditional AT with one-step Fast AT \cite{wong2020fast,andriushchenko2020understanding,zhang2022revisiting} in our training regime. This change is designed to maintain competitive unlearning performance and acceptable image utility while significantly increasing efficiency.
\textbf{Fig.\,\ref{fig: overview}} provides a performance comparison overview of our proposed DM unlearning scheme, {\ours}, against existing DM unlearning methods.

% === Contributions ===
We summarize our key \textbf{contributions} as follows:

\noindent\ding{182}
We explore the integration of AT with concept unlearning in DMs (diffusion models) and propose {\ours}. A significant challenge identified is the reduction in the utility of DMs for image generation when incorporating AT. To overcome this, we designed a utility-retaining regularization  to carefully balance the trade-off between effective unlearning and high-quality image generation.

\noindent\ding{183}
For the first time, we reveal that unlearning the text encoders within DMs can significantly enhance robustness against adversarial prompt attacks more effectively than the commonly unlearned UNet. Specifically, robustly unlearned text encoders strike a better balance between unlearning performance and image generation utility. Furthermore, a single unlearned text encoder can be shared across different DMs and can be implemented in a plug-and-play manner, greatly enhancing usability.
% Consequently, they deliver superior results in both unlearning effectiveness and maintenance of image quality compared to robust unlearned UNet. Additionally, text encoders possess plug-and-play capabilities, offering enhanced usability over UNet.

\noindent\ding{184} 
Extensive experiments validate that our approach not only achieves state-of-the-art (SOTA) unlearning performance under adversarial prompt attacks, but also preserves a commendable level of image generation utility. Additionally, we explore the use of an efficient adversarial training method, such as one-step Fast AT, as our base training scheme, which enhances training efficiency while maintaining robust unlearning and image generation utility.





==> sections/method.tex <==
% \section{Problem Statement}

% \paragraph{DM setup.} 
% %\SL{[Be consistent across paragraph titles, Setup or setup? I prefer `s'.]}
% %\yz{sure}
% The focus of our work is on latent diffusion models (LDMs) \cite{rombach2022high,cao2022survey}, which excel in the text-to-image generation task by integrating conditional text prompts---such as text-based image descriptions---into image embeddings to guide the generation process.
% In LDMs, the diffusion process initiates with a random noise sample drawn from a Gaussian distribution $\mathcal{N}(0, 1)$. This sample undergoes a progressive transformation through a series of $T$ time steps in a gradual denoising process, ultimately resulting in the creation of a clean image $\mathbf{x}$. At each time step $t$, the DM utilizes a noise estimator $\epsilon_{\boldsymbol{\theta}}(\cdot | c)$, parameterized by $\boldsymbol{\theta}$ and conditioned on an input prompt $c$, also referred to as a `concept'.
% The diffusion process operates on the latent representation $\mathbf{z}_t$ of the image at each time step. The training objective for $\boldsymbol{\theta}$ is to minimize the denoising error, which is formalized as follows:
% %\vspace*{-5mm}
% {
% \begin{align}
% \begin{array}{ll}
% \displaystyle \minimize_{\btheta}     &  \mathbb{E}_{(\mathbf x, c) \sim \mathcal D ,t, \epsilon \sim \mathcal{N}(0,1)}
% \left[
% \| \epsilon - \epsilon_{\boldsymbol \theta}(\mathbf z_t | c) \|_2^2
% \right], 
% \end{array}
% \label{eq: diffusion_training}
% \end{align}
% }%
% where $\mathcal D$ is the training set, and ${\epsilon}_{\boldsymbol{\theta}}(\mathbf{z}_t|c)$ is the LDM-associated noise estimator. 

% % ======= \paragraph{\SL{Concept-unlearned DM for safe image generation.}} =======
% \paragraph{Concept-unlearned DM for safe image generation.}
% The I2P dataset \cite{schramowski2023safe} raised safety concerns regarding current diffusion models (DMs) by collecting thousands of inappropriate prompts that could induce DMs to generate images containing harmful concepts such as `nudity'. To address this challenge, current solutions endeavor to finetune DMs for concept unlearning, which are also referred to as \textit{concept erasing} \cite{gandikota2023erasing} and \textit{concept forgetting}  \cite{zhang2023forget}. The ESD method \cite{gandikota2023erasing}, known for achieving state-of-the-art (SOTA) unlearning performance under adversarial conditions, is chosen as the foundational training scheme for our proposed unlearning scheme. In this setup, ESD employs a frozen DM to guide both conditioned and unconditioned scores, aiding finetuned DMs in forgetting specific concepts by directing outputs away from the targeted erased concept, as provided by the frozen DM. The objective function of ESD is formalized as follows:
% \begin{align}
% \minimize_{\boldsymbol{\theta}} \quad & \mathbb{E}_{c, t, \epsilon \sim \mathcal{N}(0,1)} \left[ 
% \left\| \epsilon_{\boldsymbol{\theta}}(x_{t}, c, t) - 
% \left( \epsilon_{\boldsymbol \theta^{\ast}}(x_{t}, t) - \eta \left( \epsilon_{\boldsymbol \theta^{\ast}}(x_{t}, c, t) - \epsilon_{\boldsymbol \theta^{\ast}}(x_{t}, t) \right) \right)
% \right\|_2^2 
% \right],
% \label{eq:esd}
% \end{align}
% where $\eta$ represents the negative guidance scale, $c$ refers to the descriptions of undesired concepts (e.g., `nudity'). Here, $\boldsymbol{\theta}$ denotes the model parameters of the DM being fine-tuned for concept unlearning, while $\boldsymbol{\theta}^{\ast}$ indicates the model parameters of the frozen DM used as a reference in the training process.


% % ======= \paragraph{\SL{Adversarial prompt attack against DM.}} ===========
% \paragraph{Adversarial prompt attack against DM.}
% Existing adversarial prompt attacks for unlearned DMs \cite{zhang2023generate, chin2023prompting4debugging, tsai2023ring} indicate that unlearned DMs remain susceptible to adversarial prompts. These prompts can successfully coerce DMs into generating images with supposedly unlearned concepts, highlighting a critical vulnerability. Since ESD is chosen as the base training scheme, we adopt the attack objective function inspired by ESD from \cite{chin2023prompting4debugging} to generate adversarial prompts for DMs, which leverages a frozen DM to guide the optimization direction:
% \begin{align}
% \minimize_{c^\prime} \quad & \mathbb{E}_{t, \epsilon \sim \mathcal{N}(0,1)} \left[ 
% \left\| \epsilon_{\boldsymbol{\theta}}(x_{t}, c^\prime, t) - 
% \epsilon_{\boldsymbol{\theta^{\ast}}}(x_{t}, c, t)
% \right\|_2^2 
% \right],
% \label{eq:attack}
% \end{align}
% where $c$ is the original text condition describing a scenario (e.g., `A nude lady in the bathroom.') involving concepts that DMs are trained to forget, and $c^\prime$ represents the adversarially optimized condition inputs.




% % ====== \paragraph{\SL{AdvUnlearn: An adversarial training setup of DM unlearning.}} =======
% %\SL{[introduce the generic setup of AdvUnlearn]}
% %\SL{State key questions and problems of interest: including non-trivial study of integrating AT into DM unlearning, and effective AT techniques adaptation etc.}

% \paragraph{AdvUnlearn: An adversarial training setup of DM unlearning.}
% Due to the vulnerability of unlearned DMs against adversarial prompt attacks, safety-driven unlearning transforms into a defensive mechanism in the ongoing battle between the unlearner (defender) and the attacker. To bolster the robustness of DM unlearning against adversarial attacks, a setup of adversarial training for DM unlearning ({\ours}) is urgently needed. For adversarial training (AT), adversarial input should be generated for training at each iteration. In our setting, the optimized adversarial condition inputs are created by the attacker, who directly integrates adversarially optimized continuous embeddings into the original token embeddings, bypassing the use of discrete text tokens. This approach is chosen to improve the stability and efficiency of AT for DM unlearning. Unlike attack strategies that seek specific discrete text tokens, our focus is solely on the effectiveness of the adversarial input. By optimizing directly in the embedding space, we avoid the complexities of discrete optimization, enhancing both the stability and efficiency of input generation. 
% At the start of the unlearning process, we conduct $200$ iterations of benign ESD training as a warm-up. After that, we introduce adversarial prompts into the training regimen. This process is iterative: we generate adversarial prompts $c^{\prime}$ for the most recently updated DMs using \textbf{Eq.\,(\ref{eq:attack})}, and employ these prompts for AT using \textbf{Eq.\,(\ref{eq:esd})}. As demonstrated in \cite{zhang2019theoretically}, AT would bring a trade-off between model utility and robustness in the task of image classification. The same thing would happen when AT is introduced into DM unlearning, and how to balance the trade-off between unlearning robustness and image generation quality of unlearned DMs are central to our research. 
% To address these complex issues, we explore two critical questions:
% \begin{itemize}
%   \item How to \textbf{retain image generation utility} during adversarial unlearning?
%   \item Which modules within DMs are the \textbf{best targets} for adversarial unlearning?
% \end{itemize}





% % \paragraph{Adversarial Training for DM Unlearning.}
% % The DM unlearning performance benchmark presented in \cite{zhang2023generate} indicates that unlearned DMs remain susceptible to adversarial prompts. These prompts can successfully coerce DMs into generating images with supposedly unlearned concepts, highlighting a critical vulnerability. Consequently, safety-driven unlearning transforms into a defensive mechanism in the ongoing battle between the unlearner (defender) and the attacker. To bolster the robustness of DM unlearning against adversarial attacks, integrating adversarial training (AT) is a strategic approach. 
% % The ESD method \cite{gandikota2023erasing}, known for achieving state-of-the-art (SOTA) unlearning performance under adversarial conditions, is chosen as the foundational training scheme. In this setup, ESD employs a frozen DM to guide both conditioned and unconditioned scores, aiding finetuned DMs in forgetting specific concepts by directing outputs away from the targeted erased concept, as provided by the frozen DM. The objective function of ESD is formalized as follows:
% % \begin{align}
% % \minimize_{\boldsymbol{\theta}} \quad & \mathbb{E}_{c, t, \epsilon \sim \mathcal{N}(0,1)} \left[ 
% % \left\| \epsilon_{\boldsymbol{\theta}}(x_{t}, c, t) - 
% % \left( \epsilon_{\boldsymbol \theta^{\ast}}(x_{t}, t) - \eta \left( \epsilon_{\boldsymbol \theta^{\ast}}(x_{t}, c, t) - \epsilon_{\boldsymbol \theta^{\ast}}(x_{t}, t) \right) \right)
% % \right\|_2^2 
% % \right],
% % \label{eq:esd}
% % \end{align}
% % where $\eta$ represents the guidance scale, $c$ refers to the descriptions of undesired concepts (e.g., `nudity'). Here, $\boldsymbol{\theta}$ denotes the model parameters of the DM being fine-tuned for concept unlearning, while $\boldsymbol{\theta}^{\ast}$ indicates the model parameters of the frozen DM used as a reference in the training process.
% % To generate adversarial inputs for DM, we adopt the attack objective function inspired by ESD from \cite{chin2023prompting4debugging}, which leverages a frozen DM to guide the optimization direction:
% % \begin{align}
% % \minimize_{c^\prime} \quad & \mathbb{E}_{t, \epsilon \sim \mathcal{N}(0,1)} \left[ 
% % \left\| \epsilon_{\boldsymbol{\theta}}(x_{t}, c^\prime, t) - 
% % \epsilon_{\boldsymbol{\theta^{\ast}}}(x_{t}, c, t)
% % \right\|_2^2 
% % \right],
% % \label{eq:attack}
% % \end{align}
% % where $c$ is the original text condition describing a scenario (e.g., `A nude lady in the bathroom.') involving concepts that DMs are trained to forget, and $c^\prime$ represents the adversarially optimized condition inputs. 
% % These optimized condition inputs are created by the attacker, who directly integrates adversarially optimized continuous embeddings into the original token embeddings, bypassing the use of discrete text tokens.
% % This approach is chosen to improve the stability and efficiency of adversarial training (AT) for DM unlearning. Unlike attack strategies that seek specific text tokens, our focus is 
% % % Table for Motivation
% % \begin{wraptable}{r}{65mm}
% %     %\vspace*{-7mm}
% %     \caption{\footnotesize{Performance evaluation of different unlearning methods on the UNet or text encoder of base SD-v.14 model, comparing Vanilla-ESD \cite{gandikota2023erasing} and Adv-ESD, which introduces an adversarial condition into the unlearning process. Results are measured through the Attack Success Rate (ASR) of UnlearnDiffAtk \cite{zhang2023generate}. The Fréchet Inception Distance (FID) and CLIP score are specifically averaged over $10k$ images generated based on prompts from the COCO Caption dataset \cite{chen2015microsoft}.}}
% %     %\vspace*{-4mm}
% %     \setlength\tabcolsep{4.0pt}
% %     \centering
% %     \footnotesize
% %     \resizebox{0.45\textwidth}{!}{
% %     \begin{tabular}{cc||c|cc}
% %     \toprule[1pt]
% %     \midrule
% %         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
% %           \textbf{Unlearning} \\ 
% %           \textbf{Methods}
% %         \end{tabular}} &
% %         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
% %           \textbf{Trainable} \\ 
% %           \textbf{Module}
% %         \end{tabular}} &
% %         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
% %           ASR \\ 
% %           ($\downarrow$)
% %         \end{tabular}} &
% %         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
% %           FID \\ 
% %           ($\downarrow$)
% %         \end{tabular}} &
% %         \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
% %           CLIP \\ 
% %           ($\uparrow$)
% %         \end{tabular}} \\
% %         & & & & \\
% %         \toprule
% %         -  & - & 100\% & 16.7 &  0.311 \\
        
% %         Vanilla-ESD  & UNet & 73.24\% & 18.18 &  0.302\\
% %         Vanilla-ESD  & Text Encoder & 3.52\% &  55.32 & 0.187\\
        
% %         Adv-ESD & UNet & 43.48\% & 26.48 &  0.277  \\
% %         Adv-ESD & Text Encoder & 2.82\% &  59.10 &   0.183 \\
    
% %      \midrule
% %     \bottomrule[1pt]
% %     \end{tabular}}
% %     %\vspace{-2.5mm}
% %     \label{tab: motivation}
% %     %\vspace*{-8mm}
% % \end{wraptable}
% % solely on the effectiveness of the adversarial input. By optimizing directly in the embedding space, we avoid the complexities of discrete optimization, enhancing both the stability and efficiency of input generation. This method reduces the required number of attack steps dramatically, from 3000 to just 30. However, despite these improvements, generating adversarial inputs in this way still demands more training time compared to conventional methods.
% % After $200$ steps of benign ESD training as a warm-up, we introduce adversarial prompts into the training regimen, a process we refer to as `adversarial unlearning'. This process is iterative: we generate adversarial prompts $c^{\prime}$ for the most recently updated DMs using \textbf{Eq.\,(\ref{eq:attack})}, and employ these prompts for AT using \textbf{Eq.\,(\ref{eq:esd})}. This strategy results in an adversarially unlearned DM, with performance metrics and generated image examples detailed in \textbf{Tab.\,\ref{tab: motivation}} and \textbf{Fig.\,\ref{fig: motivation}}. While AT significantly enhances the unlearning performance of UNet, it also considerably reduces the image generation utility. Moreover, the impact of the unlearning process varies significantly across different DM modules, with the text encoder particularly sensitive to these changes. Identifying the optimal module to fine-tune for unlearning purposes and balancing these trade-offs are central to our research. To address these complex issues, we explore three critical questions:
% % \begin{itemize}
% %   \item How to \textbf{retain image generation utility} during adversarial unlearning?
% %   \item Which modules within DMs are the \textbf{best targets} for adversarial unlearning?
% %   \item How can we enhance the \textbf{training efficiency} of adversarial unlearning?
% % \end{itemize}


% %

% % ====== \section{\SL{Challenge and Fix:  Maintaining Image Generation Quality in AdvUnlearn}} ====
% % \SL{[You can move some motivating results from the problem statement section.]}
% % \SL{[Clearly present the first challenge: image generation loss for direct implementation of AT, as well as your fix.]}


\section{Challenge and Fix:  Maintaining Image Generation Quality in AdvUnlearn}
% Table for Motivation
\begin{wraptable}{r}{65mm}
    \vspace*{-4mm}
    \caption{\footnotesize{Performance evaluation of different unlearning methods on the UNet or text encoder of base SD-v.14 model, comparing Vanilla-ESD \cite{gandikota2023erasing} and Adv-ESD. More metric details can be found in \textbf{Sec.\,\ref{sec: exP_setup}}}}
    %\vspace*{-4mm}
    \setlength\tabcolsep{4.0pt}
    \centering
    \footnotesize
    \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{cc||c|cc}
    \toprule[1pt]
    \midrule
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          \textbf{Unlearning} \\ 
          \textbf{Methods}
        \end{tabular}} &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          \textbf{Trainable} \\ 
          \textbf{Module}
        \end{tabular}} &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          ASR \\ 
          ($\downarrow$)
        \end{tabular}} &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          FID \\ 
          ($\downarrow$)
        \end{tabular}} &
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
          CLIP \\ 
          ($\uparrow$)
        \end{tabular}} \\
        & & & & \\
        \toprule
        -  & - & 100\% & 16.7 &  0.311 \\
        
        Vanilla-ESD  & UNet & 73.24\% & 18.18 &  0.302\\
        Vanilla-ESD  & Text Encoder & 3.52\% &  55.32 & 0.187\\
        
        Adv-ESD & UNet & 43.48\% & 26.48 &  0.277  \\
        Adv-ESD & Text Encoder & 2.82\% &  59.10 &   0.183 \\
    
     \midrule
    \bottomrule[1pt]
    \end{tabular}}
    %\vspace{-2.5mm}
    \label{tab: motivation}
    %\vspace*{-8mm}
\end{wraptable}
In text-to-image generation, similar to the trade-off between natural and robust errors in image classification as described by \cite{zhang2019theoretically}, there is a notable trade-off between unlearning efficacy and image generation utility. High unlearning efficacy implies that adversarial prompt attacks cannot compel unlearned DMs to generate images with undesired concepts. Although DM unlearning serves as a defensive mechanism, and adversarial training (AT) can enhance the robustness of DMs against such attacks, this often comes at the cost of degraded image quality, as evidenced by the results shown in \textbf{Tab.\,\ref{tab: motivation}} and \textbf{Fig.\,\ref{fig: motivation}}. To address this, we integrate loss regularization into the state-of-the-art DM unlearning method—ESD \cite{gandikota2023erasing}—aiming to balance unlearning efficacy with image generation utility. Inspired by \cite{zhang2019theoretically,stanforth2019labels, carmon2019unlabeled}, the following loss regularization on additional prompts is introduced:
\begin{align}
\minimize_{\boldsymbol{\theta}} \quad & \mathbb{E}_{t, \epsilon \sim \mathcal{N}(0,1)} \left[ 
\left\| \epsilon_{\boldsymbol{\theta}}(\mathbf x_{t} | c_{\text{retain}}) - 
\epsilon_{\btheta_\mathrm{o}}(\mathbf x_{t} | c_{\text{retain}})
\right\|_2^2 
\right],
\label{eq:loss_regularization}
\end{align}
where $c_{\text{retain}}$ refers to text prompts sampled from a dataset specifically curated for this purpose.
We construct a base dataset using the template 'a photo of [OBJECT]', where the object classes are sourced from the COCO dataset \cite{lin2014microsoft}, comprising commonly encountered objects in daily life. Subsequently, we employ a large language model (LLM) as a judger to sift through these prompts, excluding those linked to concepts designated for erasure. Detailed information about the LLM judger system is provided in \textbf{Appx.\,\ref{appx: LLM_judger}}. Our method, which integrates adversarial unlearning with loss regularization for retention, is detailed in \textbf{Alg.\,\ref{alg: pgd}}. 






%======== \section{\SL{Identifying Optimal Design Component of AdvUnlearn: Text Encoder or UNet?}} =========
%\SL{[Given that the first challenge is fixed, then clearly present the second challenge: where to conduct AT, as well as your motivating experiments, fix, and insights.]}
%\SL{[You can also mention fast AT here in order to enhance adversarial unlearning efficiency.]}

\section{Identifying Optimal Component for AdvUnlearn: Text Encoder or UNet?}

\begin{wrapfigure}{r}{85mm}
    \vspace*{-4mm}
    \centering
    \includegraphics[width=0.6\textwidth]{figs/warmup.pdf}
    \caption{\footnotesize{Visualization examples of different SD models conditioned on benign and harmful prompts. }}
    \vspace*{-4mm}
    \label{fig: motivation}
\end{wrapfigure}
With the unlearning scheme established, we next determine which module within DMs should be targeted for fine-tuning to achieve unlearning objectives. A typical text-to-image DM comprises two main components: text encoder and UNet. The text encoder processes text token embeddings to provide conditioned guidance for UNet, which predicts noises. 
As shown in \textbf{Tab.\,\ref{tab: motivation}} and \textbf{Fig.\,\ref{fig: motivation}}, the text encoder demonstrates a higher potential for achieving greater unlearning efficacy compared to UNet, even though the text encoder suffers significant image generation utility degradation due to the introduction of aggressive adversarial training (AT). Nevertheless, it is possible to find a solution to achieve a balance between image generation utility and unlearning robustness.
As previously discussed, a significant challenge in DM unlearning is the trade-off between unlearning efficacy and image generation utility. To simultaneously achieve high unlearning efficacy and maintain image generation utility, the chosen module must effectively unlearn specific concepts while minimally impacting other knowledge. According to \cite{basu2023localizing}, text encoders are more amenable to edits compared to UNet. Additionally, text encoders, having fewer parameters than UNet, can achieve convergence more rapidly. Moreover, many DMs are finetuned for various artistic tastes or functional requirements, such as those in \cite{DreamShaper, Protogen}. Typically, personalizations of DMs involve freezing the text encoder and fine-tuning only the UNet.  Therefore, a text encoder that has undergone the unlearning process with one DM can serve as a plug-in unlearner for other DMs, enhancing safety across different applications. Consequently, we select the text encoder as the target module for our proposed unlearning scheme.

Adversarial Training (AT) typically requires more time than conventional training methods, making the enhancement of training efficiency a critical focus within the field of AT. Traditionally, AT employs a multi-step attack to generate adversarial examples for training. To accelerate this process, Fast AT \cite{Wong2020Fast} introduced the use of a one-step Fast Gradient Sign Method (FGSM) attack. Following this approach, we adopt the one-step FGSM for adversarial prompt generation, which can be formalized as follows:
\begin{align}
    \delta = \delta - \alpha \cdot \text{Sign}(\nabla_{\boldsymbol{\delta}} L_2\{\epsilon_{\boldsymbol{\theta}}(x_{t},c+\delta,t), ~~\epsilon_{\boldsymbol{\theta}^{\ast}}(x_{t},c,t)\})
\end{align}
\label{eq: fast_at}








